Properties and uncertainties of scalar field models of dark energy with barotropic equation of state

The dynamics of expansion and large scale structure formation in the multicomponent Universe with dark energy modeled by the minimally coupled scalar field with generalized linear barotropic equation of state (EoS) are analyzed. It is shown that the past dynamics of expansion and future of the Universe -- eternal accelerated expansion or turnaround and collapse -- are completely defined by the current energy density of a scalar field and relation between its current and early EoS parameters. The clustering properties of such models of dark energy and their imprints in the power spectrum of matter density perturbations depend on the same relation and, additionally, on the "effective sound speed" of a scalar field, defined by its Lagrangian. It is concluded that such scalar fields with different values of these parameters are distinguishable in principle. This gives the possibility to constrain them by confronting the theoretical predictions with the corresponding observational data. For that we have used the 7-year WMAP data on CMB anisotropies, the Union2 dataset on Supernovae Ia and SDSS DR7 data on luminous red galaxies (LRG) space distribution. Using the Markov Chain Monte Carlo technique the marginalized posterior and mean likelihood distributions are computed for the scalar fields with two different Lagrangians: Klein-Gordon and Dirac-Born-Infeld ones. The properties of such scalar field models of dark energy with best fitting parameters and uncertainties of their determination are also analyzed in the paper.

==> table_1.tex <==
 \begin{table}
 \caption{The best fitting values and 1$\sigma$
 confidential ranges of cosmological parameters in the
 CSF+CDM and TSF+CDM models, determined on the base
 of WMAP7 and SDSS LRG DR7 data. The current
  Hubble parameter $H_0$ is in units km$\,$s$^{-1}\,
 $Mpc$^{-1}$, the age of the Universe $t_0$ is given 
 in Giga years.}
 \medskip
 \begin{tabular}{c|c|c}
 \hline
 & & \\
 Parameters&CSF+CDM&TSF+CDM \\
 \hline
 & & \\
$\Omega_{de}$&0.69$_{-0.08}^{+0.06}$&0.68$_{-0.08}^{+0.06}$\\
 & & \\
$w_0$&-0.80$_{-0.20}^{+0.34}$&-0.95$_{-0.05}^{+0.46}$\\
 & & \\
$c_a^2$&-0.91$_{-0.09}^{+0.91}$&-0.20$_{-0.80}^{+0.19}$\\
 & & \\
$100\Omega_b h^2$&2.27$_{-0.15}^{+0.16}$&2.27$_{-0.16}^{+0.17}$\\
 & & \\
$10\Omega_{cdm} h^2$&1.10$_{-0.13}^{+0.14}$&1.12$_{-0.15}^{+0.12}$\\
 & & \\
$H_0$&65.4$_{- 7.1}^{+ 7.0}$&65.0$_{- 7.1}^{+ 7.4}$\\
 & & \\
$n_s$&0.97$_{-0.04}^{+0.05}$&0.97$_{-0.04}^{+0.04}$\\
 & & \\
$\log(10^{10}A_s)$&3.08$_{-0.10}^{+0.09}$&3.08$_{-0.10}^{+0.09}$\\
 & & \\
$z_{rei}$&10.8$_{- 3.6}^{+ 3.2}$&10.4$_{- 3.1}^{+ 3.3}$\\
 & & \\
$\sigma_{8}$&0.75$_{-0.21}^{+0.13}$&0.74$_{-0.21}^{+0.15}$\\
 & & \\
$t_0$&13.8$_{- 0.3}^{+ 0.6}$&14.0$_{- 0.5}^{+ 0.5}$\\
 & & \\
 \hline
$-\log L$&3760.26&3760.39\\
 \hline
 \end{tabular}
 \label{tabl1}
 \end{table}


==> table_2.tex <==
 \begin{table*}
 \caption{The best fitting values and 1$\sigma$
 confidential ranges of cosmological parameters in the
 $\Lambda$CDM, CSF+CDM and TSF+CDM models determined
 on the base of complete data set listed in the
 section \ref{method_data}. The current
  Hubble parameter $H_0$ is in units km$\,$s$^{-1}\,
 $Mpc$^{-1}$, the age of the Universe $t_0$ is given 
 in Giga years.}
 \medskip
 \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
 \hline
 & & & & & & & & &\\
 Parameters&$\Lambda$CDM&CSF+CDM&TSF+CDM&CSF+CDM&
 TSF+CDM&CSF+CDM&TSF+CDM&CSF+CDM&TSF+CDM \\
 & &$w$=const&$w$=const&$c_a^2=0$&$c_a^2=0$&$c_a^2>w_0$
  &$c_a^2>w_0$&$c_a^2$ free&$c_a^2$ free\\
  &1 &2 &3 &4 &5 &6 &7 &8 &9\\
 \hline
 & & & & & & & & &\\
$\Omega_{de}$&0.72$_{-0.05}^{+0.04}$&0.72$_{-0.04}^{+0.04}$&0.72$_{-0.05}^{+0.04}$&0.72$_{-0.05}^{+0.04}$&0.72$_{-0.05}^{+0.04}$&0.71$_{-0.05}^{+0.04}$&0.71$_{-0.04}^{+0.05}$&0.72$_{-0.06}^{+0.04}$&0.72$_{-0.05}^{+0.04}$\\
 & & & & & & & & &\\
$w_0$&-1&-1.00$_{-0.00}^{+0.17}$&-0.99$_{-0.01}^{+0.16}$&-0.99$_{-0.01}^{+0.03}$&-1.00$_{-0.00}^{+0.03}$&-0.99$_{-0.01}^{+0.16}$&-1.00$_{-0.00}^{+0.17}$&-0.93$_{-0.07}^{+0.13}$&-0.97$_{-0.03}^{+0.17}$\\
 & & & & & & & & &\\
$c_a^2$&-1&-1.00$_{-0.00}^{+0.17}$&-0.99$_{-0.01}^{+0.16}$&0&0&-0.05$_{-0.94}^{+0.05}$&-0.06$_{-0.94}^{+0.06}$&-0.97$_{-0.03}^{+0.97}$&-0.99$_{-0.01}^{+0.99}$\\
 & & & & & & & & &\\
$100\Omega_b h^2$&2.27$_{-0.14}^{+0.13}$&2.25$_{-0.12}^{+0.16}$&2.26$_{-0.15}^{+0.15}$&2.26$_{-0.15}^{+0.14}$&2.24$_{-0.13}^{+0.17}$&2.25$_{-0.12}^{+0.17}$&2.25$_{-0.13}^{+0.17}$&2.25$_{-0.13}^{+0.17}$&2.29$_{-0.16}^{+0.14}$\\
 & & & & & & & & &\\
$10\Omega_{cdm} h^2$&1.14$_{-0.08}^{+0.09}$&1.15$_{-0.11}^{+0.09}$&1.14$_{-0.11}^{+0.09}$&1.14$_{-0.10}^{+0.09}$&1.14$_{-0.13}^{+0.10}$&1.13$_{-0.13}^{+0.10}$&1.15$_{-0.14}^{+0.08}$&1.11$_{-0.12}^{+0.13}$&1.13$_{-0.13}^{+0.10}$\\
 & & & & & & & & &\\
$H_0$&70.0$_{- 3.8}^{+ 3.4}$&69.4$_{- 3.9}^{+ 4.0}$&69.7$_{- 4.4}^{+ 4.0}$&69.2$_{- 4.3}^{+ 3.8}$&69.5$_{- 3.6}^{+ 4.0}$&68.6$_{- 4.4}^{+ 4.7}$&69.2$_{- 4.7}^{+ 4.2}$&69.2$_{- 5.1}^{+ 4.2}$&69.7$_{- 5.6}^{+ 3.7}$\\
 & & & & & & & & &\\
$n_s$&0.97$_{-0.03}^{+0.03}$&0.97$_{-0.03}^{+0.04}$&0.97$_{-0.04}^{+0.03}$&0.98$_{-0.04}^{+0.05}$&0.97$_{-0.03}^{+0.03}$&0.97$_{-0.04}^{+0.05}$&0.97$_{-0.03}^{+0.04}$&0.97$_{-0.03}^{+0.05}$&0.97$_{-0.04}^{+0.04}$\\
 & & & & & & & & &\\
$\log(10^{10}A_s)$&3.09$_{-0.09}^{+0.09}$&3.09$_{-0.09}^{+0.09}$&3.09$_{-0.10}^{+0.09}$&3.09$_{-0.10}^{+0.09}$&3.09$_{-0.09}^{+0.09}$&3.09$_{-0.09}^{+0.10}$&3.09$_{-0.09}^{+0.10}$&3.07$_{-0.08}^{+0.11}$&3.09$_{-0.09}^{+0.10}$\\
 & & & & & & & & &\\
$z_{rei}$&10.5$_{- 3.3}^{+ 3.0}$&10.6$_{- 3.4}^{+ 3.2}$&10.5$_{- 3.4}^{+ 3.2}$&10.7$_{- 3.3}^{+ 3.7}$&10.5$_{- 3.5}^{+ 3.2}$&10.8$_{- 3.7}^{+ 3.2}$&10.3$_{- 3.2}^{+ 3.4}$&10.3$_{- 3.3}^{+ 3.9}$&10.4$_{- 3.2}^{+ 3.4}$\\
 & & & & & & & & &\\
$\sigma_{8}$&0.83$_{-0.06}^{+0.06}$&0.83$_{-0.10}^{+0.06}$&0.83$_{-0.10}^{+0.06}$&0.78$_{-0.19}^{+0.10}$&0.82$_{-0.12}^{+0.07}$&0.78$_{-0.18}^{+0.10}$&0.83$_{-0.19}^{+0.06}$&0.79$_{-0.19}^{+0.10}$&0.81$_{-0.20}^{+0.08}$\\
 & & & & & & & & &\\
$t_0$&13.7$_{- 0.3}^{+ 0.3}$&13.8$_{- 0.3}^{+ 0.3}$&13.7$_{- 0.3}^{+ 0.3}$&13.7$_{- 0.3}^{+ 0.4}$&13.8$_{- 0.3}^{+ 0.3}$&13.8$_{- 0.4}^{+ 0.4}$&13.8$_{- 0.3}^{+ 0.4}$&13.8$_{- 0.3}^{+ 0.4}$&13.7$_{- 0.3}^{+ 0.4}$\\
 & & & & & & & & &\\
 \hline
$-\log L$&4027.60&4027.63&4027.62&4027.24&4027.75&4027.51&4027.79&4027.35&4027.41\\
 \hline
 \end{tabular}
 \label{tabl2}
 \end{table*}

